Infinite-Dimensionality in Quantum Foundations: W*-algebras as Presheaves over Matrix Algebras

In this paper, W*-algebras are presented as canonical colimits of diagrams of matrix algebras and completely positive maps. In other words, matrix algebras are dense in W*-algebras.

==> eptcsdata.tex <==
\providecommand{\firstpage}{161}
\providecommand{\publicationstatus}{R. Duncan and C. Heunen (Eds.): Quantum Physics and Logic (QPL) 2016\\
EPTCS 236, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.236.11}{10.4204/EPTCS.236.11}}
\pdfoutput=1

